Skye: A Differentiable Equation of State

Stellar evolution and numerical hydrodynamics simulations depend critically on access to fast, accurate, thermodynamically consistent equations of state. We present Skye, a new equation of state for fully-ionized matter. Skye includes the effects of positrons, relativity, electron degeneracy, Coulomb interactions, non-linear mixing effects, and quantum corrections. Skye determines the point of Coulomb crystallization in a self-consistent manner, accounting for mixing and composition effects automatically. A defining feature of this equation of state is that it uses analytic free energy terms and provides thermodynamic quantities using automatic differentiation machinery. Because of this, Skye is easily extended to include new effects by simply writing new terms in the free energy. We also introduce a novel thermodynamic extrapolation scheme for extending analytic fits to the free energy beyond the range of the fitting data while preserving desirable properties like positive entropy and sound speed. We demonstrate Skye in action in the MESA stellar evolution software instrument by computing white dwarf cooling curves.

==> Snippets/derivatives.tex <==
% $Id: derivatives.tex 385 2008-07-13 20:07:02Z efb $

%differential operators, roman typeface
\newcommand{\dif}{\ensuremath{\mathrm{d}}}
\newcommand{\Dif}{\ensuremath{\mathrm{D}}}

%derivatives
\newcommand{\D}{{\mathrm d}}
\newcommand{\DD}{{\,\D\!\!\;}}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #1}} %partialderivative 
\newcommand{\ddt}[1]{\frac{\partial #1}{\partial t}} %partial time derivative 
%\newcommand{\DDt}[1]{\frac{\dif #1}{\dif t}} %total time derivative
\newcommand{\DDt}[1]{\frac{\Dif #1}{\Dif t}} % Lagrangian time derivative
\newcommand{\ddm}[1]{\frac{\partial #1}{\partial m}} %partial derivative wrt m 
\newcommand{\ddr}[1]{\frac{\partial #1}{\partial r}} %partial derivative wrt r
\newcommand{\ddx}[1]{\frac{\partial #1}{\partial x}} %partial derivative wrt x 
\newcommand{\ddy}[1]{\frac{\partial #1}{\partial y}} %partial derivative wrt y 
\newcommand{\DDy}[1]{\frac{\dif #1}{\dif y}} %total derivative wrt y
\newcommand{\ddz}[1]{\frac{\partial #1}{\partial z}} %partial derivative wrt z 
\newcommand{\ppl}[2]{\left(\frac{\partial\ln #1}{\partial\ln
      #2}\right)_{\rho,T}}
\newcommand{\ppll}[2]{\left(\frac{\partial\ln #1}{\partial\ln
      #2}\right)_{\rho,T,\{X_{j\neq i}\}}}
\newcommand{\ddl}[2]{\frac{{\rm d}\ln #1}{{\rm d}\ln #2}}
\newcommand{\DxDy}[2]{{\frac{\D{#1}}{\D{#2}}}}
\newcommand{\dxdy}[2]{{\frac{\partial{#1}}{\partial{#2}}}}
\newcommand{\dxdyind}[3]{{\Brak{\frac{\D{#1}}{\D{#2}}}_{{#3}}}}
\newcommand{\dxdycz}[3]{{\Brak{\frac{\partial{#1}}{\partial{#2}}}_{{#3}}}}
%Misc
\newcommand{\Av}[1]{{\left\langle{#1}\right\rangle}}
\newcommand{\av}[1]{{\langle{#1}\rangle}}
\newcommand{\Frac}[2]{{\Brak{#1}/\Brak{#2}}}
\newcommand{\abs}[1]{{\left|{#1}\right|}}


==> Snippets/formatting.tex <==
%=======================================================================
%
% formatting.tex --- Formatting Macros
%
%=======================================================================

%References

\newcommand{\lSect}[1]{{\label{sec:#1}}}
\newcommand{\lFig}[1]{{\label{fig:#1}}}
\newcommand{\lEq}[1]{{\label{eq:#1}}}
\newcommand{\lTab}[1]{{\label{tab:#1}}}
\newcommand{\pFig}[1]{{\placefigure{fig:#1}}}
\newcommand{\pTab}[1]{{\placetable{tab:#1}}}
\newcommand{\Tabff}[1]{{\ref{tab:#1}}}
\newcommand{\Tab}[1]{{Table~\Tabff{#1}}}
\newcommand{\Tabs}[1]{{Tables~\Tabff{#1}}}
\newcommand{\TabRange}[2]{{Tables~\Tabff{#1} - \Tabff{#2}}}
\newcommand{\TabTwo}[2]{{Tables~\Tabff{#1} and \Tabff{#2}}}
\newcommand{\pan}[1]{{\textit{#1}}}
\newcommand{\Pan}[1]{{Panel~\pan{#1}}}
\newcommand{\Pans}[1]{{Panels~\pan{#1}}}
\newcommand{\FIGFF}[2]{{\ref{fig:#2}\pan{#1}}}
\newcommand{\Figff}[1]{{\FIGFF{}{#1}}}
\newcommand{\FIG}[2]{{Fig.~\FIGFF{#1}{#2}}}
\newcommand{\Fig}[1]{{\FIG{}{#1}}}
\newcommand{\FigTwo}[2]{{\FIGS{}{#1} and \FIGFF{}{#2}}}
\newcommand{\FIGS}[2]{{Figs.~\FIGFF{#1}{#2}}}
\newcommand{\Figs}[1]{{\FIGS{}{#1}}}
\newcommand{\Figure}[1]{{Figure~\FIGFF{}{#1}}}
\newcommand{\Figures}[1]{{Figures~\FIGFF{}{#1}}}
\newcommand{\Sectff}[1]{{\ref{sec:#1}}}
\newcommand{\Sect}[1]{{\S\Sectff{#1}}}
\newcommand{\Appendix}[1]{{Appendix~\Sectff{#1}}}
\newcommand{\Appendices}[1]{{Appendices~\Sectff{#1}}}
\newcommand{\Sects}[1]{{\S\S\Sectff{#1}}}
\newcommand{\Eqref}[1]{{\ref{eq:#1}}}
\newcommand{\Eqff}[1]{{(\Eqref{#1})}}
\newcommand{\EQ}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Equation}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Eq}[1]{{Eq.~\Eqff{#1}}}
\newcommand{\Eqs}[1]{{Eqs.~\Eqff{#1}}}
\newcommand{\Leg}[1]{{\textit{#1}}}

% formatting macros

\newcommand{\isofont}[1]{{\mathrm{#1}}}
\newcommand{\isomass}[1]{{\ensuremath{\isofont{^{#1}}}}}
\newcommand{\isocharge}[1]{{\ensuremath{\isofont{_{#1}}}}}
\newcommand{\isotope}[3]{{\ensuremath{\isocharge{#1}\isomass{#2}\isofont{#3}}}}
\newcommand{\Solar}[1]{{\ensuremath{\left[\right.}#1\ensuremath{\right.\left]}}}
\newcommand{\I}[2]{{\isotope{}{#1}{#2}}}
\newcommand{\El}[1]{{\I{}{#1}}}
\newcommand{\Rat}[4]{{\I{#1}{#2}/\I{#3}{#4}}}
\newcommand{\SolRatI}[4]{{\Solar{\Rat{#1}{#2}{#3}{#4}}}}
\newcommand{\SolI}[2]{{\Solar{\I{#1}{#2}}}} \newcommand{\SolEl}[1]{{\Solar{\El{#1}}}} 
\newcommand{\Ep}[1]{{\ensuremath{10^{#1}}}}
\newcommand{\E}[1]{{\ensuremath{\powersep\Ep{#1}}}}
\newcommand{\EE}[2]{{\ensuremath{\powersep\Ep{#1#2}}}}
\newcommand{\powersep}{\times}
\newcommand{\Brak}[1]{{\left({#1}\right)}}
\newcommand{\SBrak}[1]{{\left[{#1}\right]}}


==> Snippets/nuclides.tex <==
% $Id: nuclides.tex 385 2008-07-13 20:07:02Z efb $
% nuclides.tex
% input file with macros for nuclides

% base command
\newcommand{\nuclei}[2]{\ensuremath{\mathrm{^{#1}#2}}}

% nuclides, with most highest abundance or longest half-life as default
% for example, \carbon produces ^{12}C, \carbon[13] produces ^{13}C
%
\newcommand{\neutron}{\ensuremath{n}}
\newcommand{\nt}{\neutron}
\newcommand{\proton}{\ensuremath{p}}
\newcommand{\pt}{\proton}
\newcommand{\photon}{\ensuremath{\gamma}}
\newcommand{\hydrogen}[1][1]{\nuclei{#1}{H}}
\newcommand{\helium}[1][4]{\nuclei{#1}{He}}
\newcommand{\lithium}[1][7]{\nuclei{#1}{Li}}
\newcommand{\beryllium}[1][9]{\nuclei{#1}{Be}}
\newcommand{\boron}[1][11]{\nuclei{#1}{B}}
\newcommand{\carbon}[1][12]{\nuclei{#1}{C}}
\newcommand{\nitrogen}[1][14]{\nuclei{#1}{N}}
\newcommand{\oxygen}[1][16]{\nuclei{#1}{O}}
\newcommand{\fluorine}[1][19]{\nuclei{#1}{F}}
\newcommand{\neon}[1][20]{\nuclei{#1}{Ne}}
\newcommand{\sodium}[1][23]{\nuclei{#1}{Na}}
\newcommand{\magnesium}[1][24]{\nuclei{#1}{Mg}}
\newcommand{\aluminum}[1][27]{\nuclei{#1}{Al}}
\newcommand{\silicon}[1][28]{\nuclei{#1}{Si}}
\newcommand{\phosphorus}[1][31]{\nuclei{#1}{P}}
\newcommand{\sulfur}[1][32]{\nuclei{#1}{S}}
\newcommand{\chlorine}[1][35]{\nuclei{#1}{Cl}}
\newcommand{\argon}[1][36]{\nuclei{#1}{Ar}}
\newcommand{\potassium}[1][39]{\nuclei{#1}{K}}
\newcommand{\calcium}[1][40]{\nuclei{#1}{Ca}}
\newcommand{\scandium}[1][45]{\nuclei{#1}{Sc}}
\newcommand{\titanium}[1][48]{\nuclei{#1}{Ti}}
\newcommand{\vanadium}[1][51]{\nuclei{#1}{V}}
\newcommand{\chromium}[1][52]{\nuclei{#1}{Cr}}
\newcommand{\manganese}[1][55]{\nuclei{#1}{Mn}}
\newcommand{\iron}[1][56]{\nuclei{#1}{Fe}}
\newcommand{\cobalt}[1][59]{\nuclei{#1}{Co}}
\newcommand{\nickel}[1][58]{\nuclei{#1}{Ni}}
\newcommand{\copper}[1][63]{\nuclei{#1}{Cu}}
\newcommand{\zinc}[1][64]{\nuclei{#1}{Zn}}
\newcommand{\gallium}[1][69]{\nuclei{#1}{Ga}}
\newcommand{\germanium}[1][74]{\nuclei{#1}{Ge}}
\newcommand{\arsenic}[1][75]{\nuclei{#1}{As}}
\newcommand{\selenium}[1][80]{\nuclei{#1}{Se}}
\newcommand{\bromine}[1][79]{\nuclei{#1}{Br}}
\newcommand{\krypton}[1][84]{\nuclei{#1}{Kr}}
\newcommand{\rubidium}[1][85]{\nuclei{#1}{Rb}}
\newcommand{\strontium}[1][88]{\nuclei{#1}{Sr}}
\newcommand{\yttrium}[1][89]{\nuclei{#1}{Y}}
\newcommand{\zirconium}[1][94]{\nuclei{#1}{Zr}}
\newcommand{\niobium}[1][93]{\nuclei{#1}{Nb}}
\newcommand{\molybdenum}[1][98]{\nuclei{#1}{Mo}}
\newcommand{\technetium}[1][97]{\nuclei{#1}{Tc}}
\newcommand{\ruthenium}[1][102]{\nuclei{#1}{Ru}}
\newcommand{\rhodium}[1][103]{\nuclei{#1}{Rh }}
\newcommand{\palladium}[1][106]{\nuclei{#1}{Pd}}
\newcommand{\silver}[1][107]{\nuclei{#1}{Ag}}
\newcommand{\cadmium}[1][114]{\nuclei{#1}{Cd}}
\newcommand{\indium}[1][115]{\nuclei{#1}{In}}
\newcommand{\tin}[1][120]{\nuclei{#1}{Sn}}
\newcommand{\antimony}[1][121]{\nuclei{#1}{Sb}}
\newcommand{\tellurium}[1][130]{\nuclei{#1}{Te}}
\newcommand{\iodine}[1][127]{\nuclei{#1}{I}}
\newcommand{\xenon}[1][132]{\nuclei{#1}{Xe}}
\newcommand{\cesium}[1][133]{\nuclei{#1}{Cs}}
\newcommand{\barium}[1][138]{\nuclei{#1}{Ba}}
\newcommand{\lanthanum}[1][139]{\nuclei{#1}{La}}
\newcommand{\cerium}[1][140]{\nuclei{#1}{Ce}}
\newcommand{\praseodymium}[1][141]{\nuclei{#1}{Pr}}
\newcommand{\neodymium}[1][142]{\nuclei{#1}{Nd}}
\newcommand{\promethium}[1][147]{\nuclei{#1}{Pm}}
\newcommand{\samarium}[1][152]{\nuclei{#1}{Sm}}
\newcommand{\europium}[1][153]{\nuclei{#1}{Eu}}
\newcommand{\gadolinium}[1][158]{\nuclei{#1}{Gd}}
\newcommand{\terbium}[1][159]{\nuclei{#1}{Tb}}
\newcommand{\dysprosium}[1][164]{\nuclei{#1}{Dy}}
\newcommand{\holmium}[1][165]{\nuclei{#1}{Ho}}
\newcommand{\erbium}[1][168]{\nuclei{#1}{Er}}
\newcommand{\thulium}[1][169]{\nuclei{#1}{Tm}}
\newcommand{\ytterbium}[1][174]{\nuclei{#1}{Yb}}
\newcommand{\lutetium}[1][175]{\nuclei{#1}{Lu}}
\newcommand{\hafnium}[1][180]{\nuclei{#1}{Hf}}
\newcommand{\tantalum}[1][180]{\nuclei{#1}{Ta}}
\newcommand{\tungsten}[1][184]{\nuclei{#1}{W}}
\newcommand{\rhenium}[1][187]{\nuclei{#1}{Re}}
\newcommand{\osmium}[1][192]{\nuclei{#1}{Os}}
\newcommand{\iridium}[1][193]{\nuclei{#1}{Ir}}
\newcommand{\platnium}[1][195]{\nuclei{#1}{Pt}}
\newcommand{\gold}[1][197]{\nuclei{#1}{Au}}
\newcommand{\mercury}[1][202]{\nuclei{#1}{Hg}}
\newcommand{\thallium}[1][205]{\nuclei{#1}{Tl}}
\newcommand{\lead}[1][208]{\nuclei{#1}{Pb}}
\newcommand{\bisumth}[1][209]{\nuclei{#1}{Bi}}
\newcommand{\polonium}[1][210]{\nuclei{#1}{Po}}
\newcommand{\astatine}[1][210]{\nuclei{#1}{At}}
\newcommand{\radon}[1][222]{\nuclei{#1}{Rn}}
\newcommand{\francium}[1][223]{\nuclei{#1}{Fr}}
\newcommand{\radium}[1][226]{\nuclei{#1}{Ra}}
\newcommand{\actinium}[1][227]{\nuclei{#1}{Ac}}
\newcommand{\thorium}[1][232]{\nuclei{#1}{Th}}
\newcommand{\protactinium}[1][231]{\nuclei{#1}{Pa}}
\newcommand{\uranium}[1][238]{\nuclei{#1}{U}}
\newcommand{\neptunium}[1][237]{\nuclei{#1}{Np}}
\newcommand{\plutonium}[1][244]{\nuclei{#1}{Pu}}
\newcommand{\americium}[1][243]{\nuclei{#1}{Am}}
\newcommand{\curium}[1][247]{\nuclei{#1}{Cm}}
\newcommand{\berkelium}[1][247]{\nuclei{#1}{Bk}}
\newcommand{\californium}[1][251]{\nuclei{#1}{Cf}}
\newcommand{\einsteinium}[1][252]{\nuclei{#1}{Es}}
\newcommand{\fermium}[1][257]{\nuclei{#1}{Fm}}
\newcommand{\mendelevium}[1][258]{\nuclei{#1}{Md}}
\newcommand{\nobelium}[1][259]{\nuclei{#1}{No}}
\newcommand{\lawrencium}[1][262]{\nuclei{#1}{Lr}}
\newcommand{\rutherfordium}[1][261]{\nuclei{#1}{Rf}}
\newcommand{\dubnium}[1][268]{\nuclei{#1}{Db}}
\newcommand{\seaborgium}[1][271]{\nuclei{#1}{Sg}}
\newcommand{\bohrium}[1][274]{\nuclei{#1}{Bh}}
\newcommand{\hassium}[1][270]{\nuclei{#1}{Hs}}
\newcommand{\meitnerium}[1][278]{\nuclei{#1}{Mt}}
\newcommand{\darmstadtium}[1][281]{\nuclei{#1}{Ds}}
\newcommand{\roentgenium}[1][281]{\nuclei{#1}{Rg}}
\newcommand{\copernicum}[1][285]{\nuclei{#1}{Cn}}


==> Snippets/units.tex <==
% $Id: units.tex 385 2008-07-13 20:07:02Z efb $

%------------------------------------------------------------------------
% typesetting of units
% 
% Note that this doesn't prevent linebreaking between symbol and unit.
% A more sophisticated system is available from CTAN asa units.sty
%------------------------------------------------------------------------

% basic unit typesetteing
\newcommand{\unitspace}{\ensuremath{\,}}
\newcommand{\usp}{\unitspace}
\newcommand{\numberspace}{\ensuremath{\;}}
\newcommand{\nsp}{\numberspace}
\newcommand{\unitstyle}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\power}[2]{\ensuremath{{#1}^{#2}}}

\newcommand{\ee}[1]{\ensuremath{\times 10^{#1}}}

% prefixes
\newcommand{\nano}{\unitstyle{n}}
\newcommand{\milli}{\unitstyle{m}}
\newcommand{\centi}{\unitstyle{c}}
\newcommand{\kilo}{\unitstyle{k}}
\newcommand{\Mega}{\unitstyle{M}}
\newcommand{\Giga}{\unitstyle{G}}

% base units, mks
\newcommand{\meter}{\unitstyle{m}}
\newcommand{\kilogram}{\kilo\gram}
\newcommand{\second}{\unitstyle{s}}

\newcommand{\Kelvin}{\unitstyle{K}}
\newcommand{\K}{\Kelvin}  %degrees Kelvin

% base units, cgs
\newcommand{\cm}{\centi\meter}
\newcommand{\gram}{\unitstyle{g}}

% derived units
\newcommand{\grampercc}{\gram\usp\power{\cm}{-3}} %mass density
\newcommand{\grampersquarecm}{\gram\usp\power{\cm}{-2}} %column depth
\newcommand{\squarecmpergram}{\power{\cm}{2}\usp\power{\gram}{-1}} %opacity
\newcommand{\GramPerCc}{\grampercc}
\newcommand{\GramPerSc}{\grampersquarecm}
\newcommand{\columnunit}{\grampersquarecm}
\newcommand{\dyne}{\unitstyle{dyn}} %dyne
\newcommand{\erg}{\unitstyle{erg}} %erg 
\newcommand{\ergs}{\erg}
\newcommand{\gauss}{\unitstyle{G}} %gauss
\newcommand{\ergspersecond}{\erg\unitspace\power{\second}{-1}}
\newcommand{\ergspergram}{\erg\unitspace\power{\gram}{-1}}
\newcommand{\ergspergs}{\erg\unitspace\power{\gram}{-1}\unitspace\power{\second}{-1}} %angular momentum
\newcommand{\ergssecond}{\erg\unitspace\second}
\newcommand{\cgsflux}{\erg\unitspace\power{\cm}{-2}\usp\power{\second}{-1}}
\newcommand{\cmpersecond}{\cm\usp\power{\second}{-1}} %velocity
\newcommand{\cmpersecondSc}{\cm\usp\power{\second}{-2}} %acceleration
\newcommand{\cmSqpersecond}{\power{\cm}{2}\usp\power{\second}{-1}}%mixing

% Nuclear and atomic units
\newcommand{\amu}{\unitstyle{u}} %atomic mass unit
\newcommand{\angstrom}{\mbox{\AA}} %Angstrom
\newcommand{\fermi}{\unitstyle{fm}} %fermi
\newcommand{\eV}{\unitstyle{eV}}        %eV
\newcommand{\keV}{\kilo\eV} %Kev
\newcommand{\MeV}{\Mega\eV} %MeV

% solar and astronomical units
\newcommand{\Msun}{\ensuremath{\unitstyle{M}_\odot}}
\newcommand{\Lsun}{\ensuremath{\unitstyle{L}_{\odot}}}
\newcommand{\Rsun}{\ensuremath{\unitstyle{R}_{\odot}}}
\newcommand{\Zsun}{\ensuremath{Z_{\odot}}}
\newcommand{\Myr}{\Mega\yr}
\newcommand{\Gyr}{\Giga\yr}
\newcommand{\parsec}{\unitstyle{pc}}
\newcommand{\kpc}{\kilo\parsec} %kiloparsec
\newcommand{\mJy}{\unitstyle{\mu Jy}} %micro Jansky
\newcommand{\Msunyr}{\Msun\,\power{\yr}{-1}}
\newcommand{\MJ}{\ensuremath{\mathrm{M_J}}}
\newcommand{\RJ}{\ensuremath{\mathrm{R_J}}}
\newcommand{\Mearth}{\ensuremath{\mathrm{M_{\oplus}}}}
\newcommand{\AU}{\unitstyle{AU}}

% misc. units
\newcommand{\minute}{\unitstyle{min}} %minute
\newcommand{\hour}{\unitstyle{hr}} %hour
\newcommand{\yr}{\unitstyle{yr}}        %year
\newcommand{\km}{\kilo\meter}   %kilometers
\newcommand{\Hz}{\unitstyle{Hz}}        %Hertz
\newcommand{\ksec}{\kilo\second} %kilosecond
\newcommand{\kms}{\ensuremath{\mathrm{km}\,\second^{-1}}}
\newcommand{\vcrit}{{\varv_{\mathrm{crit}}}}
\newcommand{\vkep}{{\varv_{\mathrm{kep}}}}
\newcommand{\vsurf}{{\varv_{\mathrm{surf}}}}
\newcommand{\mol}{\unitstyle{mol}}% mole
\newcommand{\barn}{\unitstyle{b}} %barn

% command to include values
\newcommand{\unit}[2]{\ensuremath{#1\numberspace\mathrm{#2}}}


==> Snippets/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\bvec{\nabla} \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex


==> constants.tex <==
%constants
\newcommand{\kB}{\ensuremath{k_\mathrm{B}}} %Boltzmann's constant
\newcommand{\NA}{\ensuremath{N_\mathrm{\!A}}} %Avogadro number
\newcommand{\mb}{\ensuremath{m_\mathrm{u}}} %mean nucleon mas
\newcommand{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand{\alphaF}{\ensuremath{\alpha_\mathrm{F}}} %Fine structure

